Towards Automatic Evaluation and Selection of PHI De-identification Models via Multi-Agent Collaboration

Protected health information (PHI) de-identification is critical for enabling the safe reuse of clinical notes, yet evaluating and comparing PHI de-identification models typically depends on costly, small-scale expert annotations. We present TEAM-PHI, a multi-agent evaluation and selection framework that uses large language models (LLMs) to automatically measure de-identification quality and select the best-performing model without heavy reliance on gold labels. TEAM-PHI deploys multiple Evaluation Agents, each independently judging the correctness of PHI extractions and outputting structured metrics. Their results are then consolidated through an LLM-based majority voting mechanism that integrates diverse evaluator perspectives into a single, stable, and reproducible ranking. Experiments on a real-world clinical note corpus demonstrate that TEAM-PHI produces consistent and accurate rankings: despite variation across individual evaluators, LLM-based voting reliably converges on the same top-performing systems. Further comparison with ground-truth annotations and human evaluation confirms that the framework's automated rankings closely match supervised evaluation. By combining independent evaluation agents with LLM majority voting, TEAM-PHI offers a practical, secure, and cost-effective solution for automatic evaluation and best-model selection in PHI de-identification, even when ground-truth labels are limited.

==> sections/7_limitations.tex <==
\section{Limitations}

% Our study has several limitations that should be acknowledged. 

% First, the scope of evaluation is limited to a single dataset of 100 annotated clinical notes. While these notes are authentic and carefully annotated, they may not fully represent the heterogeneity of clinical documentation across institutions, specialties, and languages. As a result, our conclusions about the consistency and reliability of Evaluation Agents should be interpreted as preliminary rather than universally generalizable. Larger and more diverse corpora are needed to confirm robustness. 

% Second, our framework makes the implicit assumption that cross-agent agreement can serve as a reliable proxy for recall when ground truth is masked. This assumption may not always hold in practice, especially if multiple agents share systematic biases (e.g., under-detecting certain PHI types). In such cases, recall-proxy values could overestimate performance. The robustness of results under these assumption violations remains an open question. 

% Third, the performance of both De-id Agents and Evaluation Agents is influenced by several practical factors, including prompt design, model size, and context length. Small prompt changes or differences in tokenization may lead to variation in results. Although majority voting across Evaluation Agents helps reduce such variance, the stability of the framework is not guaranteed under all conditions. 

% Fourth, computational efficiency is a concern. Running multiple large-scale LLMs both as de-identifiers and evaluators incurs substantial costs in terms of GPU resources, latency, and energy consumption. This limits scalability for very large datasets and may not be practical for real-time or resource-constrained applications. Future work should investigate lightweight or distilled models that can approximate the same evaluation functionality at lower cost. 

% Finally, while our framework is motivated by privacy protection, it does not by itself guarantee fairness or bias mitigation. Evaluation Agents may reflect demographic or linguistic biases inherited from their training data, which could influence judgments on PHI annotation quality. Moreover, our experiments focus on PHI categories defined under U.S. regulations (HIPAA); extensions to other regulatory frameworks or languages may require adaptation and careful re-validation. 

% In summary, while the proposed framework demonstrates promise for PHI de-identification without full reliance on gold-standard annotations, its assumptions, computational demands, and limited scope of evaluation should be carefully considered when interpreting the results or deploying the system in practice.






This study has several limitations. First, evaluation was conducted on a single set of 100 annotated clinical notes, which may not capture the diversity of clinical documentation across institutions, specialties, or languages; larger and more heterogeneous datasets are needed to confirm generalizability. Second, our framework assumes that cross-agent agreement is a reliable proxy for recall when ground truth is masked. This may be violated if multiple agents share systematic biases (e.g., under-detecting specific PHI types), potentially inflating recall-proxy values. Third, performance depends on practical factors such as prompt design, model size, and context length; small prompt or tokenization changes can affect results, and while majority voting reduces variance, complete stability is not guaranteed. Fourth, deploying multiple large LLMs for both de-identification and evaluation incurs significant computational cost, which limits scalability and real-time use; lightweight or distilled models could address this. Finally, although designed for privacy protection, the framework does not inherently ensure fairness or mitigate demographic or linguistic bias, and it targets PHI categories defined under U.S. HIPAA regulations, requiring adaptation for other legal or linguistic contexts.

